Practical Anomaly Detection over Multivariate Monitoring Metrics for Online Services

As modern software systems continue to grow in terms of complexity and volume, anomaly detection on multivariate monitoring metrics, which profile systems' health status, becomes more and more critical and challenging. In particular, the dependency between different metrics and their historical patterns plays a critical role in pursuing prompt and accurate anomaly detection. Existing approaches fall short of industrial needs for being unable to capture such information efficiently. To fill this significant gap, in this paper, we propose CMAnomaly, an anomaly detection framework on multivariate monitoring metrics based on collaborative machine. The proposed collaborative machine is a mechanism to capture the pairwise interactions along with feature and temporal dimensions with linear time complexity. Cost-effective models can then be employed to leverage both the dependency between monitoring metrics and their historical patterns for anomaly detection. The proposed framework is extensively evaluated with both public data and industrial data collected from a large-scale online service system of Huawei Cloud. The experimental results demonstrate that compared with state-of-the-art baseline models, CMAnomaly achieves an average F1 score of 0.9494, outperforming baselines by 6.77% to 10.68%, and runs 10X to 20X faster. Furthermore, we also share our experience of deploying CMAnomaly in Huawei Cloud.

==> case_study/useless.tex <==
# dims = [9,10,13,14]
plt.rcParams["font.size"] = 20
plt.rcParams["font.family"] = "Times New Roman"
dims = list(range(data_dict["dim"]))[1:]
fig, ax = plt.subplots(nrows=len(dims)+1, sharey=False, figsize=(20,30))
i=0

start=300
end=-1
# ax[0].plot(recst, 'r', label='reconstruction')
# ax[0].legend(loc='best')
for i in range(len(dims)):
    j = dims[i] 
    ax[i].plot(recst_list[start:end, j].reshape(-1), 'r', label='Prediction'.format(i), alpha=0.3)
    ax[i].plot(real_list[start:end, j].reshape(-1), 'steelblue', label='Observation'.format(i), alpha=1)
#     ax[i].plot(diff_list[0:, j].reshape(-1), 'g', label='KPI Error Score')
#     ax[i].plot(window_dict["test_labels"][0:, -1].reshape(-1)*0.2+0.4, 'brown', label='Label')
    ax[i].legend(loc=(0.01, 0.68), prop={"size":23})
    ax[i].set_ylim([0,1.1])
ax[-1].plot(((score_dict["score"]-0.5) * 10)[start:end], label='Entity Anomaly Score')
ax[-1].set_ylim([0.4,1])
# ax[-1].plot(((diff_list))[start:end], label='Entity error score')


# ax[-1].plot(([(best_theta-0.5)*10+0.1] * len(score_dict["score"]))[start:end], label='Threshold')
# ax[-1].plot((window_dict["test_labels"][0:, -1].reshape(-1)*0.3)[start:end], 'brown', label='Label')
# ax[-1].set_ylim([0.8,1])
# ax[1].legend(loc='best')

plt.legend(loc=(0.01, 0.78), prop={"size":23})
# plt.suptitle("Result of the autoencoder")
# plt.show()
plt.savefig("./case_study.pdf")
